Stochastic Zeroth Order Gradient and Hessian Estimators: Variance Reduction and Refined Bias Bounds

We study stochastic zeroth order gradient and Hessian estimators for real-valued functions in $\mathbb{R}^n$. We show that, via taking finite difference along random orthogonal directions, the variance of the stochastic finite difference estimators can be significantly reduced. In particular, we design estimators for smooth functions such that, if one uses $ \Theta \left( k \right) $ random directions sampled from the Stiefel's manifold $ \text{St} (n,k) $ and finite-difference granularity $\delta$, the variance of the gradient estimator is bounded by $ \mathcal{O} \left( \left( \frac{n}{k} - 1 \right) + \left( \frac{n^2}{k} - n \right) \delta^2 + \frac{ n^2 \delta^4 }{ k } \right) $, and the variance of the Hessian estimator is bounded by $\mathcal{O} \left( \left( \frac{n^2}{k^2} - 1 \right) + \left( \frac{n^4}{k^2} - n^2 \right) \delta^2 + \frac{n^4 \delta^4 }{k^2} \right) $. When $k = n$, the variances become negligibly small. In addition, we provide improved bias bounds for the estimators. The bias of both gradient and Hessian estimators for smooth function $f$ is of order $\mathcal{O} \left( \delta^2 \Gamma \right)$, where $\delta$ is the finite-difference granularity, and $ \Gamma $ depends on high order derivatives of $f$. Our results are evidenced by empirical observations.

==> figures.tex <==

% This section lists additional figures. 

\begin{figure}[h]
    \centering
    \subfloat[$ x = 0, \delta = 0.1, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x0_delta01_k100.png}}
    \subfloat[$ x = 0, \delta = 0.1, k = 200 $]{\includegraphics[width = 0.45\textwidth]{grad_x0_delta01_k200.png}} \\
    \subfloat[$ x = 0, \delta = 0.01, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x0_delta001_k100.png}}
    \subfloat[$ x = 0, \delta = 0.01, k = 200 $]{\includegraphics[width =  0.45\textwidth]{grad_x0_delta001_k200.png}} \\ 
    \subfloat[$ x = 0, \delta = 0.001, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x0_delta0001_k100.png}}
    \subfloat[$ x = 0, \delta = 0.001, k = 200 $]{\includegraphics[width = 0.45\textwidth]{grad_x0_delta0001_k200.png}} 
    % \subfloat[$ x = 0, \delta = 0.1, k = 300 $]{\includegraphics[scale = 0.4]{grad_x0_delta0.1_k300.png}} \hfill
    % \subfloat[$ x = 0, \delta = 0.1, k = 400 $]{\includegraphics[scale = 0.4]{grad_x0_delta0.1_k400.png}} 
    \caption{Errors of $ \wh{\nabla} f_k^\delta (x) $, $ \wh{\nabla} f_{k,B}^\delta (x) $, $ \wh{\nabla} f_{k,G}^\delta (x) $, $ \wh{\nabla} f_{k,R}^\delta (x) $ on test function (Eq. \ref{eq:test}). Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See caption of Figure \ref{fig:grad-compare-main} for detailed illustration. 
    }
    % , on different values of $(x, \delta, k)$. \label{fig:grad-compare-supp1}}
\end{figure} 



\begin{figure}[h] 
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta01_k100.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 200 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta01_k200.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta001_k100.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 200 $]{\includegraphics[width =  0.45\textwidth]{grad_x1_delta001_k200.png}} \\ 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 100 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta0001_k100.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 200 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta0001_k200.png}} 
    \caption{Errors of $ \wh{\nabla} f_k^\delta (x) $, $ \wh{\nabla} f_{k,B}^\delta (x) $, $ \wh{\nabla} f_{k,G}^\delta (x) $, $ \wh{\nabla} f_{k,R}^\delta (x) $ on test function (Eq. \ref{eq:test}). Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See caption of Figure \ref{fig:grad-compare-main} for detailed illustration. 
    }
    % , on different values of $(x, \delta, k)$. \label{fig:grad-compare-supp1}}
\end{figure} 



\begin{figure}[h] 
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 300 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta01_k300.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 400 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta01_k400.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 300 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta001_k300.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 400 $]{\includegraphics[width =  0.45\textwidth]{grad_x1_delta001_k400.png}} \\ 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 300 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta0001_k300.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 400 $]{\includegraphics[width = 0.45\textwidth]{grad_x1_delta0001_k400.png}} 
    \caption{Errors of $ \wh{\nabla} f_k^\delta (x) $, $ \wh{\nabla} f_{k,B}^\delta (x) $, $ \wh{\nabla} f_{k,G}^\delta (x) $ on test function (Eq. \ref{eq:test}). Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See caption of Figure \ref{fig:grad-compare-main} for detailed illustration. 
    }
    % , on different values of $(x, \delta, k)$. \label{fig:grad-compare-supp1}}
\end{figure} 


\begin{figure}
    \centering
    \subfloat[$ x = 0, \delta = 0.1, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta01_k100.png}} 
    \subfloat[$ x = 0, \delta = 0.1, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta01_k200.png}} \\
    \subfloat[$ x = 0, \delta = 0.01, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta001_k100.png}} 
    \subfloat[$ x = 0, \delta = 0.01, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta001_k200.png}} \\
    \subfloat[$ x = 0, \delta = 0.001, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta0001_k100.png}} 
    \subfloat[$ x = 0, \delta = 0.001, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x0_delta0001_k200.png}} 
    \caption{Cosine similarity between the gradient estimation and the true gradient, using the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See the caption of Figure \ref{fig:grad-compare-main2} for detailed illustration.} 
\end{figure} 



\begin{figure}
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta01_k100.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta01_k200.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta001_k100.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta001_k200.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 100 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta0001_k100.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 200 $]{\includegraphics[scale = 0.45]{grad_comp_x1_delta0001_k200.png}} 
    \caption{Cosine similarity between the gradient estimation and the true gradient, using the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See the caption of Figure \ref{fig:grad-compare-main2} for detailed illustration.} 
\end{figure} 


\begin{figure}
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 300 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta01_k300.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 400 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta01_k400.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 300 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta001_k300.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 400 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta001_k400.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 300 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta0001_k300.png}} 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 400 $]{\includegraphics[width = 0.48\textwidth]{grad_comp_x1_delta0001_k400.png}} 
    \caption{Cosine similarity between the gradient estimation and the true gradient, using the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See the caption of Figure \ref{fig:grad-compare-main2} for detailed illustration.} 
\end{figure} 


\begin{figure}[h] 
    \centering
    \subfloat[$ x = 0, \delta = 0.1, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x0_delta01_k20.png}}
    \subfloat[$ x = 0, \delta = 0.1, k = 40 $]{\includegraphics[width = 0.48\textwidth]{hess_x0_delta01_k40.png}} \\
    \subfloat[$ x = 0, \delta = 0.01, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x0_delta001_k20.png}}
    \subfloat[$ x = 0, \delta = 0.01, k = 40 $]{\includegraphics[width =  0.48\textwidth]{hess_x0_delta001_k40.png}} \\ 
    \subfloat[$ x = 0, \delta = 0.001, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x0_delta0001_k20.png}}
    \subfloat[$ x = 0, \delta = 0.001, k = 40 $]{\includegraphics[width = 0.48\textwidth]{hess_x0_delta0001_k40.png}} 
    \caption{Errors of Hessian estimators on the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See the caption of Figure \ref{fig:hess-compare-main} for detailed illustration. 
    \label{fig:hess-compare-app0}}
\end{figure} 



\begin{figure}[h]
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta01_k20.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 40 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta01_k40.png}} \\ 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta001_k20.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 40 $]{\includegraphics[width =  0.48\textwidth]{hess_x025pi_delta001_k40.png}} \\ 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 20 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta0001_k20.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 40 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta0001_k40.png}} 
    \caption{Errors of Hessian estimators on the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. This figure shows that when $k$ is much smaller than $n$, $\wh{\H} f_{k,S}^\delta (x)$ \citep{wang2022hess} can achieve same level of accuracy as $ \wh{\H} f_k^\delta (x) $. See the caption of Figure \ref{fig:hess-compare-main} for detailed illustration. 
    \label{fig:hess-compare-app1}}
\end{figure} 

\begin{figure}[h]
    \centering
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 60 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta01_k60.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.1, k = 80 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta01_k80.png}} \\
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 60 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta001_k60.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.01, k = 80 $]{\includegraphics[width =  0.48\textwidth]{hess_x025pi_delta001_k80.png}} \\ 
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 60 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta0001_k60.png}}
    \subfloat[$ x = \frac{\pi}{4} \mathbf{1}, \delta = 0.001, k = 80 $]{\includegraphics[width = 0.48\textwidth]{hess_x025pi_delta0001_k80.png}} 
    \caption{Errors of Hessian estimators on the test function defined in (Eq. \ref{eq:test}). 
    Each subfigure corresponds to a different combination of the location for estimation $x$, the finite difference granularity $ \delta $, and number of random directions $k$. See the caption of Figure \ref{fig:hess-compare-main} for detailed illustration. 
    \label{fig:hess-compare-app2}}
\end{figure} 

==> maybeuseful.tex <==

\begin{proof} 

    % \textcolor{red}{revise this proof.} 
    
    We say that $ \texttt{GS}(n,k) $ is a $k$-Gram-Schmit sampling process over $\S^{n-1}$. 
    Note that $ \texttt{GS}(n,k) $ (Algorithm \ref{alg:gram-schmidt}) returns $k$ $(k \le n)$ vectors $v_1, v_2, \cdots, v_k$ from $ \S^{n-1} $. 
    % For any $k$ ($1 \le k \le n$), let $v_1, v_2, \cdots v_k$ be sampled from the Gram-Schmit sampling process over $ \S^{n-1} $. Note that 
    Conditioning on any  $ v_i $ ($1\le i \le k \le n$), the vectors $ v_1, \cdots, v_{i-1}, v_{i+1}, \cdots, v_k $ are sampled over $  \S^{n-1} \cap \{ v_i \}^{\perp} \cong \S^{n-2} $, effectively following a $(k-1)$-Gram-Schmit sampling process over $ \S^{n-2} $. 
    
    Note that the Hausdorff measure with respect to the Euclidean inner product on $\text{St} (n,k)$ is rotation-invariant. 
    By uniqueness of Haar measure on the orthogonal group, the rotation-invariant measure on $\text{St} (n,k)$ is unique. Thus the Hausdorff measure is the unique (up to constant scaling) rotation-invariant measure over Stiefel's manifolds $\text{St} (n,k)$, for any given $k$ ($1\le k \le n$). 
    Let $ \Pr $ denote the probability density functions of $ v_i $'s with respect to the Hausdorff measure (of proper dimension). 
    % We automatically switch to Lebesgue measure of a proper subspace for marginal densities. 
    
    We first show that the joint densities are constant. For any $j$ ($1\le j \le k-1$), conditioning on any $ v_1, v_2, \cdots, v_j $, the sampling process for $v_{j+1}, v_{j+2}, \cdots, v_k$ is a $(k-j)$-Gram-Schmidt sampling process over $ \S^{n-1} \cap \(\mathrm{span}\{ v_1, v_2, \cdots, v_j \} \)^\perp \cong \S^{n - 1 - j} $. Thus we have 
    \begin{align*} 
        \Pr \( v_1, v_2, \cdots, v_k \) 
        =& \;  
        \Pr \(v_2, v_3 \cdots, v_k | v_1 \)  \Pr \( v_1 \) \\
        =& \;  
        \cdots \\ 
        =& \;  
        \Pr \(v_k | v_1, v_2, \cdots, v_{k-1} \) \cdots \Pr \(v_2 | v_1 \) \Pr \( v_1 \) \\
        =& \; 
        \frac{1}{ \prod_{j=1}^n A_{n+1-j} } > 0,  
    \end{align*}
    where $A_m$ is the surface area of $\S^{m-1}$. 
    % , and the last line uses the rotation-invariance of $ \mathcal{N} (0,I) $ to compute the conditional densities. 
    
    
    
    
    Next we show that the marginal densities are constant. 

    % For $ i = 1$, the statement is trivially true. 
    
    % For $i \ge 2$, assume the following induction hypothesis: The joint density for the Gram-Schmidt sampling process of $i-1$ vectors is constant. 
    
    Fix any $i $ ($1\le i \le k$). Conditioning on any fixed $ v_1 $, the sampling process for $v_2, v_3, \cdots, v_i$ is a $(k-1)$-Gram-Schmidt sampling process over $ \S^{n-1} \cap \{ v_1 \}^\perp \cong \S^{n-2} $. On the other hand, conditioning on any fixed $ v_i $, the sampling process for $v_1, v_2, \cdots, v_{i-1}$ is a $(k-1)$-Gram-Schmidt sampling process over $ \S^{n-1} \cap \{ v_i \}^\perp \cong \S^{n-2} $. As shown above, the joint density for the Gram-Schmit sampling process is constant, which implies $ \Pr \( v_i, v_{i-1}, \cdots, v_2 | v_1 \) = \Pr \( v_{i-1}, v_{i-2}, \cdots, v_1 | v_i \) $. 
    
    Thus we have, for any $ v_i, v_{i-1}, v_{i-2}, \cdots, v_1 $, 
    \begin{align*}
        \Pr \( v_i, v_{i-1}, \cdots, v_1 \) 
        =& \; 
        \Pr \( v_i, v_{i-1}, \cdots, v_2 | v_1 \) \Pr \( v_1 \) \\ 
        =& \; 
        \Pr \( v_{i-1}, v_{i-2}, \cdots, v_1 | v_i \) \Pr \( v_1 \) \\ 
        =& \; 
        \frac{ \Pr \( v_i , v_{i-1}, v_{i-2}, \cdots, v_1 \) }{ \Pr \( v_i \) } \Pr \( v_1 \) , 
    \end{align*} 
    which implies $ \Pr \( v_i \) = \Pr \( v_1 \) $, since $ \Pr \( v_i , v_{i-1}, v_{i-2}, \cdots, v_1 \) $ is strictly positive. 
    % We can conclude the proof since the Hausdorff measure over $ \S^{n-1} $ 
    This implies that the marginal density for $ v_i $ is constant. 
    
    % In addition, we have 
    % \begin{align*} 
    %     \Pr ( v_1, v_2, \cdots, v_i ) = \Pr ( v_2, \cdots, v_i | v_1 ) \Pr (v_1), 
    % \end{align*} 
    % which is constant, since $ \Pr ( v_2, \cdots, v_i | v_1 ) $ and $\Pr (v_1) $ are constants. This means that the induction hypothesis is true for $i$ as well. 
    
\end{proof} 
